Tight High Probability Bounds for Linear Stochastic Approximation with Fixed Stepsize

This paper provides a non-asymptotic analysis of linear stochastic approximation (LSA) algorithms with fixed stepsize. This family of methods arises in many machine learning tasks and is used to obtain approximate solutions of a linear system $\bar{A}\theta = \bar{b}$ for which $\bar{A}$ and $\bar{b}$ can only be accessed through random estimates $\{({\bf A}_n, {\bf b}_n): n \in \mathbb{N}^*\}$. Our analysis is based on new results regarding moments and high probability bounds for products of matrices which are shown to be tight. We derive high probability bounds on the performance of LSA under weaker conditions on the sequence $\{({\bf A}_n, {\bf b}_n): n \in \mathbb{N}^*\}$ than previous works. However, in contrast, we establish polynomial concentration bounds with order depending on the stepsize. We show that our conclusions cannot be improved without additional assumptions on the sequence of random matrices $\{{\bf A}_n: n \in \mathbb{N}^*\}$, and in particular that no Gaussian or exponential high probability bounds can hold. Finally, we pay a particular attention to establishing bounds with sharp order with respect to the number of iterations and the stepsize and whose leading terms contain the covariance matrices appearing in the central limit theorems.

==> DesiredResults.tex <==
We consider linear stochastic optimization with and without averaging, and obtain optimal concentration rates for three noise types: almost surely contractive, almost surely bounded, and with finite moments. More precisely we consider the iterations
\begin{equation} \label{eq:lsa}
    \theta_{t+1} = \theta_t - \alpha \{ \funcA{\State_{t+1}}  \theta_t - \funcb{\State_{t+1}} \},~~t \geq 0\,,
\end{equation}
where $\alpha > 0$ is a (constant) step-size, and $\funcA{\State_{t+1}}$ (resp. $\funcb{\State_{t+1}}$) are i.i.d. random matrices (resp. i.i.d. random vectors), and independent of each other. Moreover, the random vectors $\funcb{\State_{t+1}}$ are $\sigma_b$-sub-Gaussian. Finally, we denote as $\bar{\theta}_t = \frac{1}{t}\sum_{i<t}\theta_i$ the average of the iterates.
\subsection{Linear stochastic approximation without averaging}
\begin{theorem}
Let $\delta\in(0,1]$. Then, with probability $1-\delta$,
\begin{equation}
\|\theta_T - \theta^*\| \leq q_{1-\delta,\infty} + \Delta_{RM}(T,\delta)\,,
\end{equation}
where $q_{1-\delta,\infty} = \lim_{t\to +\infty} q_{1-\delta}(\theta_t - \theta^*)$ is the limit $(1-\delta)$-quantile of the iterates, and $\Delta_{RM}(T,\delta)$ is defined as follows:
\begin{enumerate}
\item \textbf{Contractive case:} If $\exists \varepsilon > 0$ such that $\|\funcA{\State_1} - A\|_Q \leq (1 - \varepsilon - \|I - \alpha A\|_Q)/\alpha$ almost surely, then
\begin{equation}
\Delta_{RM}(T,\delta) = O\left(\frac{\sqrt{\log(1/\delta)}}{T^a}\right)\,.
\end{equation}
\item \textbf{Bounded case:} If $\|\funcA{\State_1} - A\|_Q \leq B$ almost surely and $B > (1 - \|I - \alpha A\|_Q)/\alpha$, then
\begin{equation}
\Delta_{RM}(T,\delta) = O\left(\frac{\sqrt{\log(1/\delta)} + e^{-bT + c\sqrt{T\log(d/\delta)}}}{T^a}\right)\,.
\end{equation} 
\item \textbf{Finite moments case:} If $\mathbb{E}\left[\|\funcA{\State_1} - A\|_Q^p\right] \leq C^p$, then
\begin{equation}
\Delta_{RM}(T,\delta) = O\left(\frac{1}{T^a \delta^b}\right)\,.
\end{equation}
\end{enumerate}
The constants need to be made explicit, but you get the idea...
\end{theorem}




==> Markov.tex <==
\subsection{Uniformly Geometrically Ergodic MC}
\begin{theorem}
\label{th:general_expectation UGE}
    Consider a sequence of random matrices $(\Y_\ell)_{\ell \geq 0} \in \rset^{d \times d}$. Let \(\mathfrak{F}_k = \sigma\{ \Y_{\ell}, \ell \le k\}\) and \(\PE_k [\xi] = \PE[\xi \vert \mathfrak{F}_k]\).  Assume that there exists deterministic $m_\ell \in (0,1), \sigma_\ell > 0$ such that \(\norm{\PE_{\ell-1}[\Y_\ell]}[Q]^2  \leq 1 - m_\ell\) and \(\norm{\Y_\ell - \PE_{\ell-1}[\Y_\ell]}[Q]  \leq \sigma_\ell\) almost surely for all \(\ell \geq 1\). Form a product
    \[
        Z_n = \prod_{\ell = 0}^n \Y_\ell.
    \]
    Then for any $2 \le q \le p$,
    \[
        \norm{Z_n}[p,q] \leq \sqrt{\qcond} \rme^{- \sum_{\ell=1}^n m_\ell + C_p \sum_{\ell=1}^n \sigma_\ell^2} \norm{f_Q(Z_0)}[p, q].
    \]
\end{theorem}
\begin{proof}[Proof of Theorem~\ref{th:general_expectation} ]
    We note that
    \[
        \norm{Z_n}[p,q] \leq \sqrt{\qcond} \norm{f_Q(Z_n)}[p,q].
    \]
    Consider the following decomposition:
    \[
        Z_n = \Y_n \cdot Z_{n-1} = (\Y_n - \PE_{n-1}[ \Y_n]) Z_{n-1}+ \PE_{n-1}[\Y_n] Z_{n-1} = A_n + B_n. 
    \]
    Since \(\PE[A_n \vert B_n] = \PE[f_Q(A_n) \vert f_Q(B_n)] = 0\), we can apply Proposition \ref{prop:subquadratic} and obtain the following bound:
    \[
        \norm{f_Q(Z_n)}[p,q]^2 \leq \norm{f_Q(B_n)}[p,q]^2 + C_p \norm{f_Q(A_n)}[p,q]^2. 
    \]
    Applying \eqref{eq: BX inequality} and \(\norm{\Y_n - \PE_{n-1}[\Y_n]}[Q]  \leq \sigma_n\)
    \begin{align*}
        \norm{f_Q(A_n)}[p,q] &= \left(\PE\left[ \norm{ f_Q(\Y_n - \PE_{n-1}[ \Y_n])  f_Q(Z_{n-1})}[p]^q \right]\right)^{1/q} \leq\\
        &\leq \left(\PE\left[ \normop{f_Q(\Y_n - \PE_{n-1}[ \Y_n])}^q \norm{f_Q(Z_{n-1})}[p]^q \right]\right)^{1/q} =\\
        &=  \left(\PE\left[ \normop{\Y_n - \PE_{n-1} [\Y_n]}[Q]^q  \norm{f_Q(Z_{n-1}}[p]^q  \right]\right)^{1/q} \leq\sigma_n \cdot \norm{ f_Q(Z_{n-1})}[p,q].
    \end{align*}
   Similarly, using \eqref{eq: BX inequality}  and $\norm{\PE_{n-1}[\Y_n]}[Q]^2  \leq 1 - m_n$
    \begin{align*}
        \norm{f_Q(B_n)}[p,q]^2 &= \left(\PE\left[ \norm{ f_Q(\PE_{n-1}[\Y_n])  f_Q(Z_{n-1})}[p]^q \right]\right)^{2/q} \leq\\
        &\leq \left(\PE\left[ \normop{f_Q(\PE_{n-1}[ Y_n])}^q  \norm{f_Q(Z_{n-1}) }[p]^q \right]\right)^{2/q} =\\
        &=  \left(\PE\left[ \norm{\PE_{n-1}[ Y_n]}[Q]^q \norm{f_Q(Z_{n-1})}[p]^q \right]\right)^{2/q} \leq (1 - m_n)^2 \norm{f_Q(Z_{n-1})}[p,q]^2.
    \end{align*}
    The last two inequalities imply
    \begin{align*}
        \norm{f_Q(Z_n)}[p,q]^2 &\leq ((1 - m_n)^2 + C_p\sigma_n^2)  \norm{f_Q(Z_{n-1})}[p,q]^2.
    \end{align*}
    Iteratively repeating this calculations and using \(1+x \leq \rme^x\) we come to the following estimate
     \begin{align*}
        \norm{f_Q(Z_n)}[p,q]^2  \leq \exp\left(-\sum_{i=1}^n m_i + C_p \sum_{i=1}^n \sigma_i^2\right) \cdot \Vert f_Q(Z_0) \Vert_{p,q}^2.
    \end{align*}
\end{proof}
Set
$$
\alpha_\infty = (1/2) \normop{A}[Q]^{-2} \normop{Q}^{-1} \wedge (a/4)(\kappa \bConst{A})^{-2} \rme^{-a}
$$
\begin{Prop}
Let $(Z_\ell)_{\ell \geq 1}$ satisfies  and $\alpha_\ell \in (0, \alpha_\infty)$. Then for any $2 \le q \le p$,
\begin{equation}
 \label{eq:concentration UGE}  \norm{Z_n}[p,q] \leq \kappa \exp\left( - \frac{ah}{4}\sum_{i=1}^{n/h} \alpha_{(i-1)h+1} + 9 b_Q^2 h^2 C_p \sum_{i=1}^{n/h} \alpha_{(i-1)h+1}^2 \right) d^{1/p}. 
\end{equation}
\end{Prop}
\begin{proof}
First note that for any $z_0 \in \msz$, by the Markov property,
\begin{equation}
  \label{proof:main_theo_1_markov_use}
\PE_{z_0}[ \normop{\ProdB_{m+1:n}}^{p}]  = \PE_{z_0}[ \normop{\ProdB_{m+1:n}(Z_{m+1:n})}^{p}]  = \PE_{z_0}[ \PE_{\State_m}[ \normop{\ProdB_{m+1:n}(Z_{1:n-m})}^{p} ] \eqsp.
\end{equation}
The first step is to fix some value $\State_m = z_m \in \msz$ and to derive a bound on $\PE_{z_m}[ \normopLigne{\ProdB_{m+1:n}(Z_{1:n-m})}^{p}]$. We denote by $\myqcond= \qcond^{\half}$ where $\qcond$ is defined in \eqref{eq: Lyapunov eq}.
% Consider a block length $h\in\nset$  and define the sequence $j_0 =m, \, j_{\ell+1} = \min(j_\ell + h, n)$ such that $j_{\ell+1} - j_{\ell} \le h$. Let $N= \ceil{(n-m)/h}$, where $\ceil{\cdot}$ is the ceiling function so that $j_{\ell} = j_N =n$ for any $\ell \geq N$
Consider a block length $h\in\nset$. Let $N= \ceil{(n-m)/h}$, where $\ceil{\cdot}$ is the ceiling function. Define the sequence $j_0 =m, \, j_1 = (n - m) - h N, j_{\ell} = j_{\ell-1} + h, \ell = 2, N$. Then, we introduce the decomposition
\begin{equation}
  \label{eq:decomp_Gamma_proof_main}
 \ProdB_{m+1:n}(Z_{1:n-m}) = \prod_{\ell=1}^N \BlockB_{\ell} \quad \text{where} \quad \BlockB_{\ell} :=
\prod_{i=j_{\ell-1}+1}^{j_\ell} (\Id_d - \alpha_i
\funcA{\State_{i-m}}), ~~\ell \in \{1,\ldots,N\} \eqsp.
  \end{equation}
Set $\Y_\ell = \BlockB_{\ell+1}, \ell = 0, \ldots, N-1$. Using that $(Z_k)_{k \in\nset}$ satisfies
($\mathsf{UGE}$), it can be shown that if $h$ is sufficiently large,
then $\BlockB_{\ell}$ is  close in $\mathrm{L}^p$ to the deterministic matrix
$\BlockDet_{\ell} = \prod_{i=j_{\ell-1}+1}^{j_\ell} (\Id_d - \alpha_i
A)$. 
To apply Theorem \ref{th:general_expectation} we need to calculate $m_\ell$ and $\sigma_\ell$. Let $\PE_{\ell}[\cdot] = \PE[\cdot\vert \State_{j_{\ell} - m} ]$.
\begin{lemma}
    There exist $h$ given in such that for any $\ell = 2, \ldots, N$,
    \[
        \norm{\PE_{\ell-1}[ \BlockB_{\ell}]}[Q]^2 \leq 1 - \alpha_{j_{\ell-1}+1} \frac{ah}{4}.
    \]
\end{lemma}
\begin{proof}
We may decompose the difference $\BlockB_{\ell}$  as follows:
\begin{equation} \label{eq:split_main}
    \BlockB_{\ell}  = \Id_d - \alpha_{j_{\ell-1}+1} h A   - S_\ell  + R_\ell + \bar{R}_\ell \eqsp,
\end{equation}
where $S_{\ell} = \sum_{k = j_{\ell-1}+1}^{j_{\ell}}\alpha_{k}\bigl\{\funcA{\State_{k-m}} - A\bigr\}$ is  linear ($r=1$) and the  remainders collect the higher-order terms ($r \geq 2$) in the products
\vspace{-.1cm}
\begin{equation} \label{eq:RlRlbar_def}
    \bar{R}_{\ell} = \sum_{r=2}^{h}(-1)^{r}\sum_{(i_1,\dots,i_r)\in\msi_r^\ell}\prod_{u=1}^{r}\alpha_{i_u}\funcA{\State_{i_u-m}}, ~ R_{\ell} = \sum_{k = j_{\ell-1}+1}^{j_{\ell}}(\alpha_{j_{\ell-1}+1} - \alpha_{k}) A  
    \vspace{-.1cm}
\end{equation}
where we have set  $\msi_r^{\ell} = \{(i_1,\ldots,i_r) \in \{j_{\ell-1}+1,\ldots,j_{\ell}\}^r\, : \, i_1 < \cdots < i_r \}$. It is straightforward to check that
\begin{equation}
    \norm{\bar{R}_{\ell}}[Q] \le \sum_{r=2}^{h} (\alpha_{j_{\ell-1}+1} \kappa \bConst{A} )^r \binom{h}{r}  \le  (\kappa \bConst{A} \alpha_{j_{\ell-1}+1} h)^2  (1 + \kappa \bConst{A} \alpha_{j_{\ell-1}+1})^{h}/2.
\end{equation}
Using 
\begin{align*}
        \norm{\PE_{\ell-1}[S_\ell]}[Q]  &\leq \kappa \sum_{k = j_{\ell-1}+1}^{j_{\ell}}\alpha_{k} \normop{\PE_{\ell-1}[\funcA{\State_{k-m}} - A]} \\
        &\leq \kappa \sum_{k = j_{\ell-1}+1}^{j_{\ell}}\alpha_{k} \sqrt{\sum_{\ell_1, \ell_2=1}^d \left( \PE_{\ell-1}[\bar A_{\ell_1, \ell_2}(\State_{k-m}) - A_{\ell_1, \ell_2}]\right)^2  } \\
        &\leq 
        d \kappa \bConst{A} \varsigma \sum_{k = j_{\ell-1}+1}^{j_{\ell}}\alpha_{k} \rho^{k - j_{\ell-1}} \le \frac{d \kappa \bConst{A} \rho \varsigma \alpha_{j_{\ell-1}+1} }{1 - \rho}.
    \end{align*}
The last bounds imply that
\begin{align*}
    \norm{\PE_{\ell-1}[ \BlockB_{\ell}]}[Q] \le \norm{\Id_d -  \alpha_{j_{\ell-1}+1} h A}[Q] + \frac{d \kappa \bConst{A} \varsigma \alpha_{j_{\ell-1}+1} }{1 - \rho} + (\kappa \bConst{A} \alpha_{j_{\ell-1}+1} h)^2  (1 + \kappa \bConst{A} \alpha_{j_{\ell-1}+1})^{h}/2.
\end{align*}
We have $\alpha_{j_{\ell-1}+1} h \le \alpha_{\infty} h \le (1/2) \normop{A}[Q]^{-2} \normop{Q}^{-1} \wedge (a/4)(\kappa \bConst{A})^{-2} \rme^{-a}$. By Lemma \ref{lem:Hurwitzstability} we get
\begin{align*}
    \norm{\PE_{\ell-1}[ \BlockB_{\ell}]}[Q] \le 1 -  (a/2) \alpha_{j_{\ell-1}+1} h + \frac{d \kappa \bConst{A} \varsigma \alpha_{j_{\ell-1}+1} }{1 - \rho} + (a/8) \alpha_{j_{\ell-1}+1} h .
\end{align*}
We choose $h \geq 8 d \kappa \bConst{A} \varsigma /(a (1 - \rho)) $.
\end{proof}








    

Our next goal is to bound the conditional variance term.
\begin{lemma}
    There is a such choice of \(h\), such that
    \[
        \norm{\BlockB_{\ell} - \PE_{\State_{j_{\ell-1}}}[ \BlockB_{\ell}]}[Q] \leq () \alpha_{j_{\ell-1}+1} h
    \]
    almost surely for all \(\ell \geq 1\).
\end{lemma}
\begin{proof} 
Using \eqref{eq:split_main} and bound 
\begin{align*}
\norm{\BlockB_{\ell}] - \PE_{\State_{j_{\ell-1}}}[ \BlockB_{\ell}]}[Q] &\leq \sum_{k = j_{\ell-1}+1}^{j_{\ell}}\alpha_{k} \norm{\funcA{\State_k} - \PE_{\State_{j_{\ell-1}}}[\funcA{\State_k}]}[Q] \\
&+ (\kappa \bConst{A} \alpha_{j_{\ell-1}+1} h)^2  (1 + \kappa \bConst{A} \alpha_{j_{\ell-1}+1})^{h} \\
& \le (2 \kappa \bConst{A} + (a/4) ) \alpha_{j_{\ell-1}+1} h. 
\end{align*}
\end{proof}
 
\end{proof}


\subsection{High-probability bounds}
It is easy to see that both \eqref{concentration iid} and may be rewritten in the following way. There exist constants $c_1, c_2 > 0$ such that
$$
 \norm{Z_n}[p,q] \leq \sqrt{\qcond} d^{1/p} \rme^{ - c_1 \sum_{\ell=1}^n \alpha_\ell + c_2 C_p \sum_{\ell=1}^n \alpha_\ell^2}.
$$
Denote by \(S_n = \sum_{k=1}^n \alpha_k, \nu^2_n = \sum_{k=1}^n \alpha^2_k\). Then, we take $p = q$ and use Markov's inequality
\begin{align*}
    \Pr[ \normop{Z_n} > t \sqrt{\qcond} \rme^{-c_1 S_n}] &\leq \inf_{p \geq 2} t^{-p}  \E[\normop{Z_n}^p] \qcond^{-p/2} \rme^{p c_1 S_n} \leq \inf_{p \geq 2} t^{-p}\cdot \norm{Z_n}[p,p]^p \qcond^{-p/2} \rme^{p c_1 S_n} \leq\\\
    &\leq d \inf_{p \geq 2} \left( \exp\left( c_2 p^2  \nu^2_n \right)  t^{-p}\right) =\\
    &=d \inf_{p \geq 2} \left(\exp\left( c_2 p^2  \nu^2_n - p \log t \right)\right) = d \exp \left( -\frac{\log^2 t}{ 4 c_2\nu^2_n} \right).
\end{align*}
We get the following result. 
\begin{Prop}
Assume that there exists constants $c_1, c_2 > 0$ such that for any $2 \le q \le p$
$$
\norm{Z_n}[p,q] \leq \sqrt{\qcond} d^{1/p} \rme^{ - c_1 \sum_{\ell=1}^n \alpha_\ell + c_2 C_p \sum_{\ell=1}^n \alpha_\ell^2}.
$$
Then for any $\delta \in (0,1)$ with probability at least $1 - \delta$,
$$
\normop{Z_n} \le   \sqrt{\qcond} \rme^{-c_1 S_n + 2 \nu_n \sqrt{c_2 \log(d/\delta)}}. 
$$
\end{Prop}

Given a function $g$ on $\Theta \times \Zset$ we set 
\begin{equation}
    \label{eq:definition-normLip}
    \normlip{g}= \sup_{ \theta \neq \theta', x \in \Zset} \frac{\|g(\theta,x) - g(\theta',x)\|}{\|\theta - \theta'\|}
\end{equation}
and $\lipspace{\Theta \times \Xset}= \{ g; \normlip{g} < \infty\}$.
\begin{theorem}
Assume  \Cref{assum:uge}, \Cref{assum:Abounded}, and \Cref{assum:Hurwitzmatrices}. There exist a constant $\Const{\lip}$ such that,  for any  $g \in \lipspace{\Theta \times \Xset}$, 
\begin{equation}
|\PE_{\theta_0,z}[g(\theta_n,Z_n)] - \PE_{\theta'_0,z'}[g(\theta_n,Z_n)]| \leq \Const{\lip} \rho^n \normlip{g}.     
\end{equation}
\end{theorem}
\begin{proof}
The proof uses a coupling argument. We denote by $P$ the Markov kernel governing $\{Z_n\}$. We assume for simplicity that there exists $\varepsilon > 0$ such that, for all $z \in \Zset$, 
\begin{equation}
\label{eq:one-step-minoration}
P(z,\cdot) \geq \varepsilon \nu \eqsp, 
\end{equation}
where $\varepsilon > 0$. We will deal with $m$-step minoration later. 
Define the residual kernel
\begin{equation}
\label{eq:residual-kernel}
R(z,\cdot)= (1-\epsilon)^{-1} (P(z,\cdot)-\epsilon\nu)
\end{equation}
At each iteration of the algorithm  
At each iteration of the algorithm, we couple $(Z_n,Z'_n)$ as follows. 
If $(Z_k,Z'_k)=(z,z')$, then
\begin{itemize}
\item if $z=z'$, then $Z_{k+1}$ is sampled  from  the distribution
  $P(z,\cdot)$, independently of the past. Set then $Z'_{k+1}=Z_{k+1}$;
\item If $z \ne z'$, a coin is tossed with probability of heads $\epsilon$.
\begin{itemize}
\item If the coin comes up heads, then $Z_{k+1}$ is sampled from the distribution $\nu$ and we set
  $Z'_{k+1}=Z_{k+1}$.
\item If the coin comes up tails, then  $Z_{k+1}$ and $Z'_{k+1}$ are sampled independently of each other
  and from the past from the residual kernels $R(z,\cdot)$ and
  $R(z',\cdot)$, respectively.
\end{itemize}
\end{itemize}
We then set 
\begin{align}
\theta_{k+1}&= (\Id- \gamma \funcA{Z_{k+1}}) \theta_k + \gamma \funcb{Z_{k+1}} \eqsp, \\
\theta'_{k+1}&= (\Id- \gamma \funcA{Z'_{k+1}}) \theta'_k + \gamma \funcb{Z'_{k+1}} \eqsp.
\end{align}
The associated coupling kernel may be written as 
\begin{multline}
K(z_0,\theta_0,z'_0,\theta'_0;\rmd( z_1,\theta_1,z'_1,\theta'_1))= 
\Big\{ \epsilon \bar{\nu}(\rmd (z_1,z'_1)) \\
+ (1-\epsilon) 
R(z_0,\rmd z_1) \otimes R(z'_0, \rmd z'_1) \Big\}
\delta_{F_{z_1}(\theta_0}(\rmd \theta_1) \otimes \delta_{F_{z'_1}(\theta'_0}(\rmd \theta'_1)
\end{multline}
where we have denoted $\bar{\nu}(\rmd (z_1,z'_1))= \nu(\rmd_{z_1}) \delta_{z_1}(\rmd z'_1)$ and
\begin{equation}
\label{eq:definition-F}
F_z(\theta)= (\Id - \gamma \funcA{z}) \theta + \gamma \funcb{z} \eqsp.
\end{equation}
It is easily seen that $K$ is a kernel coupling of
\end{proof}


We may use \cite[Theorem 4.1]{pinelis_1994} to get
\begin{multline}
\label{eq:pinelis_J_n_1}
\PE[ \bigl|u^\top J_{n}^{(1)}\bigr|^p ] \leq \underbrace{\alpha^{2p} (\bConst{\sf{Rm},1}  p)^{p/2} \PE \Bigl [ \sum_{\ell=1}^{n-1}\PE_{\ell+1:n}[(u^\top S_{\ell+1:n} \funnoise{\State_\ell})^2]\Bigr]^{p/2}}_{T_1}  \\+ \underbrace{\alpha^{2p}  \bConst{\sf{Rm},2}^p p^p \PE[\{\max_\ell |u^\top S_{\ell+1:n}\funnoise{\State_\ell}|\}^p]}_{T_2}\eqsp, 
\end{multline}
where $\bConst{\sf{Rm},1}, \bConst{\sf{Rm},2}$ are the constants in \cite[Theorem 4.1]{pinelis_1994}. Denote $V_{\ell+1}^\top = u^\top S_{\ell+1:n}$. To bound $T_1$, we apply the Minkowski inequality and obtain
\begin{align*}
&\PE^{2/p} \Bigl [ \sum_{\ell=1}^{n-1}\PE_{\ell+1:n}[(V_{\ell+1}^\top \funnoise{\State_\ell})^2]\Bigr]^{p/2} \le\sum_{\ell=1}^{n-1} \PE^{2/p}[\PE_{\ell+1:n}[(V_{\ell+1}^\top \funnoise{\State_\ell})^2]]^{p/2} \\
& \qquad\qquad\qquad \leq \sum_{\ell=1}^{n-1} \PE^{2/p}[\norm{\Gamma_\noise^{1/2} V_{\ell+1}}^{p}] \leq \norm{\Gamma_\noise} \sum_{\ell=1}^{n-1}\PE^{2/p}[\norm{V_{\ell+1}}^p]\eqsp.
\end{align*}
Note that by Assumption \ref{assum:Abounded} and Lemma~\ref{lem:Hurwitzstability}, $\norm{(\Id - \alpha A)^{n-k-1} \funcAt{\State_k} (\Id - \alpha A)^{k-1 - \ell}} \leq \qcond \bConst{A}(1-\alpha a)^{(n-\ell-2)/2}$. Applying Hoeffding inequality for Hilbert space-valued martingales (\cite[Theorem~3.5]{pinelis_1994}),
\begin{align*}
\PP\biggl(\norm{V_{\ell+1}} \geq \sqrt{2\bConst{A}^2 \qcond^2\log(2/\delta)(n-\ell)(1-\alpha a)^{(n-\ell-2)}}\biggr) \leq \delta\eqsp.
\end{align*}
It is easy to transform this bound into $L_p$ bound \alex{Check!}
\begin{equation}
\label{eq:l_p_bound_V_ell}
\PE^{2/p}[\norm{V_{\ell+1}}^p] \leq p (2\sqrt{2})  \bConst{A}^2\qcond^2(n-\ell)(1-\alpha a)^{(n-\ell-2)}.
\end{equation} 
The last inequality implies,
\[
T_1 \le \alpha^{p} p^p \sfD_3^p \quad \text{where} \quad \sfD_3 = 2 \bConst{\sf{Rm},1}^{1/2}  \bConst{A} \qcond \norm{\Gamma_\noise}^{1/2} a^{-1} (1 - a \alpha)^{-1} \eqsp.
\]
Now we bound the term $T_2$. Since $S_{\ell+1:n}$ and $\funnoise{\State_\ell}$ are independent, 
$$
\PE[|u^\top S_{\ell+1:n}\funnoise{\State_\ell}|^p] \leq \PE [\normop{V_{\ell+1}}^p] \sup_{u \in S^{d-1}} \PE[|u^\top\funnoise{\State_\ell}|^p ]\,.
$$
Assumption \Cref{assum:b_subexp} and Lemma \ref{lem: pmomSG} imply, that for any $u \in S_{d-1}$,
\begin{align*}
\PE[|u^\top\funnoise{\State_\ell}|^p ] \leq p^{p/2} \bConst{\beps}^p (2 \sqrt 2)^{p/2}  
\eqsp.
\end{align*}
Combining this bound with \eqref{eq:l_p_bound_V_ell},
\begin{align*}
\PE[|u^\top S_{\ell+1:n}\funnoise{\State_\ell}|^p] &\leq p^{p} (2\sqrt{2})^{p}   \bConst{A}^p\qcond^p \bConst{\beps}^p (n-\ell)^{p/2}(1-\alpha a)^{(n-\ell-2)p/2}.,
\end{align*}
We can obtain the following bound for $T_2$
\begin{align*}
    T_2 &\le \alpha^{2p} p^{2p} (2\sqrt{2})^{p}   \bConst{A}^p\qcond^p \bConst{\beps}^p \bConst{\sf{Rm},2}^p  \sum_{\ell=1}^{n-1} (n-\ell)^{p/2}(1-\alpha a)^{(n-\ell-2)p/2} \\
    &\le \alpha^{2p} p^{2p} (2\sqrt{2})^{p}   \bConst{A}^p\qcond^p \bConst{\beps}^p \bConst{\sf{Rm},2}^p  \Bigg ( \sum_{\ell=1}^{n-1} (n-\ell)(1-\alpha a)^{(n-\ell-2)} \Bigg)^{p/2} \\
    &\le \alpha^p \sfD_4^p p^{2p}, \quad \text{where} \quad \sfD_4 = (2 \sqrt 2) \bConst{A} \qcond \bConst{\beps} \bConst{\sf{Rm},2} (1 - \alpha a)^{-1} a^{-1}.
\end{align*}
Finally,
$$
\PE[ \bigl|u^\top J_{n}^{(1)}\bigr|^p ] \leq \alpha^p p^{2p} (\sfD_3 + \sfD_4)^p. 
$$

Using Markov's inequality we get with probability at least $1 - \delta$,
$$
\bigl|u^\top J_{n}^{(1)}\bigr| \leq \ConstD_{1} \alpha \log(1/\delta) + \ConstD_{2} \alpha^{3/2} (\log{n})^{3/2}\log^{5/2}(1/\delta)\eqsp.  
$$

==> Rosenthal.tex <==
\subsection{Rosenthal inequality for Markov chains}
In this section, we provide a general weighted Rosenthal inequality for Markov chains with kernel $\MK$ with certain contractivity properties in Wasserstein distance. In addition, we apply this result to obtain bounds which will be useful in the proof of our main results. We state the following assumptions
\begin{assumR}
\label{assG:kernelP_q}
There exist a measurable function $V: \msx \to [1,\infty)$, $\lambda \in (0,1)$ and $b < \infty$ such that for any $x \in \msx$, $\MK V(x) \leq \lambda V(x) + b$.
\end{assumR}

\begin{assumR}
\label{assG:kernelP_q_smallset}
Moreover, there exist an integer $ m \geq 1$, $\epsilon \in (0,1)$ and $d>0$ such that the level set
  $\{V(x) \leq d\}$ is $(m,\epsilon)$-small and $\lambda+2b/(1+d)<1$.
\end{assumR}

\begin{proposition}
Under \Cref{assG:kernelP_q} and \Cref{assG:kernelP_q_smallset}  the Markov kernel $\MK$ admits a unique invariant probability measure $\pi$, $\pi(V) < \infty$ and for all probability measures $\xi$ such that $\xi(V) < \infty$ and $n \geq 1$,
\begin{align}
    \label{eq:V-geometric-coupling-general}
    \tvnorm{\xi \MK^n - \pi} \leq \Vnorm[V]{\xi \MK^n - \pi} \leq c_m \{ \xi(V) + \pi(V) \} \rho^n \eqsp,
  \end{align}
  where the constants $\rho, \bar\lambda_m, \bar{b}_m$ are given by
  \begin{equation}
    \label{eq:bornes-v-geometric-coupling}
      \begin{aligned}
        \log\rho & = \frac{\log(1-\epsilon) \log\bar\lambda_m} { m\bigl(\log(1-\epsilon) +
          \log\bar\lambda_m-\log\bar{b}_m\bigr) } \eqsp ,\\
        \bar\lambda_m & = \lambda^m+2b_m/(1+d) \eqsp,
        \eqspp \bar{b}_m = \lambda^m b_m + d
        \eqsp, \eqspp b_m=b (1-\lambda^m) /(1-\lambda) \eqsp ,   \\
        c_m  &= \rho^{-m}\{\lambda^m+(1-\lambda^m)/(1-\lambda)\}\{1+\bar{b}_m/[(1-\epsilon)(1-\bar\lambda_m)]\} \eqsp.
  \end{aligned}
\end{equation}
\end{proposition}
\begin{proof}
  See~\cite[Theorem~19.4.1]{douc:moulines:priouret:soulier:2018}.
\end{proof}

\begin{assumR}
\label{assG:kernelP_q_contractingset_m}
There exist a kernel coupling $\MKK$ of $\MK$, $m \in \nset, \varepsilon \in (0,1)$, $\vartheta \geq 1$ and $d > 0$ such that $\lambda+2b/(1+d)<1$, $\MKK \metricc(x,x') \leq \vartheta \metricc(x,x')$ and
\begin{equation}
\label{eq:wasserstein_contraction_m_steps}
\MKK^m \metricc(x,x') \leq (1 - \varepsilon \indi{\bar C})\metricc(x,x')
\end{equation}
for $(x, x') \in \bar C = \{V(x) \leq d\} \times \{V(x') \leq d\}$. Here $\lambda, b$ are defined in \Cref{assG:kernelP_q}.
\end{assumR}

%Check R3 assumption
\begin{lemma}
Consider the Markov chain $\theta_{n+1} = \bigl(\Id - \alpha \funcAw_{n+1}\bigr)\theta_n + \alpha \funcbw_{n+1}$ and denote the corresponding Markov kernel by $\MK$. Consider $\metricc(\theta,\theta') = \norm{\theta-\theta'}$ for $\theta,\theta' \in \rset^d$. Then there exists such $m \in \nset$, that \eqref{eq:wasserstein_contraction_m_steps} holds with $\bar C = \rset^{2d}$.
\end{lemma}
\begin{proof}
Let us fix arbitrary $\theta,\theta' \in \rset^d$. Define the sequences
\begin{align*}
\begin{cases}
\theta_{n} = \bigl(\Id - \alpha \funcAw_{n}\bigr)\theta_{n-1} + \alpha \funcbw_{n}\eqsp, n \geq 1, \eqsp \theta_{0} = \theta\eqsp;\\
\theta_{n}^{\prime} = \bigl(\Id - \alpha \funcAw_{n}\bigr)\theta_{n-1}^{\prime} + \alpha \funcbw_{n}\eqsp, n \geq 1, \eqsp \theta_{0}^{\prime} = \theta'\eqsp.\\
\end{cases}
\end{align*}
It is easy to see that $(\theta_{n},\theta_{n}^{\prime})$ is a coupling for $(\MK^n,\MK^n)$, and for any $n \geq 1$,
\begin{align*}
\MKK^{n}\norm{\theta-\theta'} = \PE[\norm{\theta_{n}-\theta_{n}^{\prime}}] = \PE[\norm{\bigl(\Id - \alpha \funcAw_{n}\bigr)(\theta_{n-1}-\theta_{n-1}^{\prime})}]\eqsp.
\end{align*}
Hence, proceeding by induction,
\begin{align*}
\MKK^{n}\norm{\theta-\theta'} = \PE\bigl[\normop{\prod_{k=1}^{n}\bigl(\Id - \alpha \funcAw_{k}\bigr)(\theta-\theta^{\prime})}\bigr] \leq \qcond (1-\alpha a/2)^{n/2}\norm{\theta-\theta^{\prime}}\eqsp.
\end{align*}
Hence, $\eqref{eq:wasserstein_contraction_m_steps}$ holds with 
\begin{align*}
m = \inf\{n \geq 1: \qcond (1-\alpha a/2)^{n/2} \leq 1-\varepsilon\} = \left\lceil \frac{2\log{(1-\varepsilon)/\qcond}}{\log{(1-\alpha a /2)}}\right\rceil\eqsp.
\end{align*}
\end{proof}

%Check R1 assumption
\begin{lemma}
Let $\alpha \in (0,\alpha_{\infty} \wedge a/(2b_Q^2(p_0-1)))$ and let $V(\theta) = \norm{\theta}^{2p}$. Then it holds
\[
\MK^{m} V(\theta) \leq \lambda_{p} V(\theta) + b_{p}\eqsp,
\]
where $m = $, $\lambda_p = $, $b_{p} = $.
\end{lemma}
\begin{proof}
Using the definition of the Markov kernel $\MK$ and Minkowski's inequality,
\begin{align*}
\MK^{m} V(\theta) = \PE\bigl[\norm{\Gamma_{1:m}\theta + \alpha\sum_{\ell=1}^{m}\Gamma_{\ell+1:m}\funcbw_{\ell}}^{2p}\bigr] \leq \left(\PE^{1/(2p)}\bigl[\norm{\Gamma_{1:m}\theta}^{2p}\bigr] + \alpha\sum_{\ell=1}^{m}\PE^{1/(2p)}\bigl[\norm{\Gamma_{\ell+1:m}\funcbw_{\ell}}^{2p}\bigr]\right)^{2p}\eqsp.
\end{align*}
Using \Cref{corr:concentration iid} together with the independence of $\Gamma_{\ell+1:m}$ and $\funcbw_{\ell}$, we obtain
\begin{align*}
\PE^{1/(2p)}\bigl[\norm{\Gamma_{1:m}\theta}^{2p}\bigr] 
&\leq \qcond d^{1/(2p)} (1 - a \alpha + (2p-1) b_Q^2 \alpha^2)^{m/2} \norm{\theta} \\
&\leq \qcond d^{1/(2p)} (1-\alpha a /2)^{m/2} \norm{\theta}\eqsp,
\end{align*}
where the last line follows from $\alpha < a/(2b_Q^2(p_0-1))$. Similarly, 
\begin{align*}
\PE^{1/(2p)}\bigl[\norm{\Gamma_{\ell+1:m}\funcbw_{\ell}}^{2p}\bigr] 
&\leq \qcond d^{1/(2p)}(1-\alpha a /2)^{(m-\ell)/2} \PE^{1/(2p)}[\norm{\funcbw_{\ell}}^{2p}] \\
&\leq 16\qcond (\sqrt{2}\rme d)^{1/(2p)}(1-\alpha a /2)^{(m-\ell)/2}\sqrt{2/e}\sqrt{2p}\sqrt{6}d^{1/2}\bConst_{b}\eqsp,
\end{align*}
where in the last inequality we have used \Cref{lem:norm_subgaus_vector} and \cref{lem: pmomSG}.
Combining the previous bounds and using the inequality $(a+b)^{2p} \leq \rme a^{2p} + p^{p}b^{2p}$ for $a>0,b>0$, 
\begin{align*}
\MK^{m} V(\theta) \leq \rme d \qcond^{2p} (1-\alpha a/2)^{mp}\norm{\theta}^{2p} + C_0^{2p}d^{p+1}p^{2p}\eqsp,
\end{align*}
where 
$$
C_0 = \frac{64\sqrt{3}\qcond \bConst{b}}{a}\eqsp.
$$



\end{proof}

Let $\bar V(x,x') = \{V(x) + V(x')\}/2$.
\begin{proposition}
\label{prop:wasser:geo}
Let \Cref{assG:kernelP_q} and \Cref{assG:kernelP_q_contractingset_m} hold.  Then the Markov kernel $P$ admits a unique invariant probability measure $\pi$, $\pi(V) < \infty$. Furthermore, for all $\alpha \in (0,1)$, $(x,x')\in \msx^2$, $p \le 2q$, and $n\in \nset$, $n \geq m$ it holds that
\begin{equation}
\label{eq: constraction}
\PE_{x,x'}^{\MKK}[\metricc^{1-\alpha}(X_n, X_n') \bar V^{\alpha p/(2q)}(X_n, X'_n)] \leq \kappa \vartheta_{\alpha}^{p/(2q)} \bar V^{\alpha p/(2q)}(x,x') \metricc^{1-\alpha}(x,x') \rho_{\alpha}^{np/(2q)}  \eqsp.
\end{equation}
Here
\begin{equation}
      \label{eq:def:rho}
      \rho_{\alpha}  = \Bigl(\frac{\bar \lambda_m \bar{d}+\delta_{\alpha}}{\bar{d}+\delta_{\alpha}} \Bigr)^{\alpha/m} < 1,  \quad \vartheta_{\alpha} = (1 + b/(1-\lambda) + \delta_{\alpha})^\alpha / \rho_\alpha^m, \quad \kappa = \vartheta^{m(1 - \alpha)} \eqsp,
    \end{equation}
$\delta_{\alpha}$ is the unique positive root of
    \begin{equation}
    \label{eq: delta def}
     (1-\epsilon)^{(1-\alpha)/\alpha} \left(\frac{\bar \lambda_m+ b_m+\delta}{1+\delta}\right) =  \frac{\bar \lambda_m \bar{d}+\delta}{\bar{d}+\delta}\eqsp,
    \end{equation}
and  $\bar \lambda_m = \lambda^m+ 2 b_m/(1+d), b_m = b(1-\lambda^m)/(1-\lambda)$ and  $\bar d = (d+1)/2$.
\end{proposition}
\begin{proof}
Existence of invariant distribution $\pi$ follows from~\cite[Theorem~20.2.1]{douc:moulines:priouret:soulier:2018}. The proof of~\eqref{eq: constraction} is postponed to~\Cref{sec:proof-ros_W_q}.
\end{proof}

For any $f: \msx \to \rset$ we define
\begin{equation*}
\Nnorm[\alpha, q, V]{f} := \max \bigg \{\sup_{x \neq x' \in \msx^2} \frac{|f(x) - f(x')|}{\metricc^{1-\alpha}(x,x') \bar V^{\alpha/(2q)}(x,x')} , \, \sup_{x \in \msx} \frac{|f(x)|}{V^{\alpha/(2q)}(x)} \bigg\} \eqsp.
\end{equation*}
Denote by $\mathcal L_{\alpha, q, V} := \{f: \msx \to \rset: \Nnorm[\alpha, q, V]{f} < \infty\}$.

\begin{theorem}
\label{th:Rosenthal_w_contracting}
Let \Cref{assG:kernelP_q} and \Cref{assG:kernelP_q_contractingset_m} hold and $q \in (1,\infty)$. Let $(g_{\ell})_{\ell = 0}^{n-1} \in \Lclass_{\alpha, q,V}$. Then, for any probability measure $\xi$ such that $\xi(V^\alpha )<\infty$,
\begin{equation}
\begin{split}
    \PE_\xi[|S_n|^{2q}] &\le \rme \momentGq[q] \{\PVar[\pi](S_n)\}^q+ \rme (8 \kappa)^{2q}  \{\pi(V^\alpha)\}^{q+1}  \vartheta_\alpha^{q} \sum_{u=1}^{q-1} B_{u,q} G_{n,q}^{u} M_q^{2(q-u)} \\
    & +  \vartheta_\alpha M_q^{2q} (2q+1)^{2q} \left( \xi(V^\alpha) + \pi(V^\alpha) \right) (1 - \rho_{\alpha}^{1/2q})^{-2q} \eqsp,
\end{split}
\end{equation}
where $G_{n,q} = \sum_{\ell=0}^{n-1}\Nnorm[\alpha, q,V]{\bar g_i}^2$, $M_q = \max_{\ell = 0, \ldots, n-1} \Nnorm[\alpha, q,V]{\bar g_i}$, $B_{u,q}$ is defined as
\begin{equation}
\label{eq: B_u_q_def}
    B_{u,q} = \frac{q!}{u!}\biggl(\frac{1}{\rho}\biggr)^{u}\biggl(\frac{2}{\log{1/\rho}}\biggr)^{2q-u}\sum_{k_1 + \ldots + k_u = 2q, k_i \geq 2}  \prod_{i=1}^u (k_{i}!)^2 \eqsp,
\end{equation}
and $\rho_{\alpha}, \kappa$ are defined in \eqref{eq:def:rho}.
\begin{remark}
Expression $B_{u,q}$ can be upper bounded as 
\[
B_{u,q} \leq \frac{q!}{u!} \biggl(\frac{2}{\log{1/\rho}}\biggr)^{2q-u}\biggl(\frac{1}{\rho}\biggr)^{u} \binom{2q-u-1}{u-1} \bigl((2q-2u+2)!\bigr)^2 2^{2u-2}\eqsp, 1 \leq u \leq q-1\eqsp.
\]
The details are given in \Cref{lem:A_B_bound}.
\end{remark}
\end{theorem}


\subsection{A fundamental identity and a key lemma}

Let $W$ be a $n$-dimensional random vector. Denote by $\varphi_W$ its characteristic function defined for any $u \in \rset^n$ by $\varphi_W(u) =\PE[\rme^{\rmi \ps{u}{W}}]$. Let $\bnu= (\nu_1,\dots, \nu_n) \in \nset^n$. If $\PE[\prod_{i=1}^n |W_i|^{\nu_i}] < \infty$, define the mixed cumulant of $W$ by
\[
\Gamma_{\bnu}(W)=\left.\frac{1}{\rmi^{|\nu|}} \frac{\partial^{|\bnu|}}{\partial u_{1}^{\nu_{1}} \ldots \partial u_{n}^{\nu_{n}}} \ln \varphi_W(u) \right|_{u=0} \eqsp,
\]
where $|\bnu| = \nu_1 + \ldots + \nu_n$. If $\nu_1=\dots=\nu_n=1$, we simply denote $\Gamma(W)= \Gamma_{\bnu}(W)$. 
Set $Z_{{n+1}} = 1$ and define $Z_{\ell}$, for $\ell= n, \dots, 2$ by the backward recursion
\begin{equation}
  \label{eq:def_Z_i_center_moment}
  Z_{{\ell}} = W_{\ell} Z_{{\ell+1}} - \PE[ W_{\ell} Z_{{\ell+1}}]\eqsp.
\end{equation}
Define the centered moment of $W$ by
\begin{equation}
\label{eq:def_centered_moment}
  \PEC[W] = \PE[W_1 Z_{2}],
\end{equation}

For any ordered subset $I =(i_1,\ldots,i_k) \subset \{1,\ldots,n\}^k$, $W_I$ stand for the $k$-dimensional random variable $(W_{i_1},\ldots,W_{i_k})$. \cite[Lemma 3]{Statul1970} allows to express cumulants in terms of centered moments:
\begin{equation}
    \label{eq:cumulantsviamoments}
    \Gamma(W) = \sum_{\nu=1}^k (-1)^{\nu-1} \sum\nolimits_{\bigcup_{p=1}^\nu I_p = I} N_\nu(I_1, \ldots, I_\nu) \prod_{p=1}^\nu \PEC[W_{I_p} ] \eqsp,
\end{equation}
where  $N_\nu(I_1,\dots,I_\nu)$ are non-negative integers defined in \cite[Appendix~2]{saulis:statulevicius:1991} and $\sum_{\bigcup_{p=1}^\nu I_p = I}$ denotes the summation over the family $ \{I_1,\ldots,I_\nu\}$  such that there exists a partition $J_1,\ldots,J_\nu$ of $\{1,\ldots,k\}$ satisfying for any $\ell \in \{1,\ldots,\nu\}$, $I_\ell = (i_{j_1},\ldots,i_{j_{n_\ell}})$ with $J_{\ell} = \{j_1,\ldots,j_{n_{\ell}} \}$, $j_1 < \ldots < j_{n_{\ell}}$. It is shown in  \cite[Corollary Lemma~4.3]{saulis:statulevicius:1991}
that
\begin{equation}
\label{eq:formula-summation}
\sum_{\nu=1}^k \sum\nolimits_{\bigcup_{p=1}^\nu I_p = I} N_\nu(I_1, \ldots, I_\nu)  = (k-1)! \eqsp.
\end{equation}
 Consider $g_\ell \in \mrl^{n}_{V^{1/2q}}$, $\ell \in \{0, \ldots, n-1\}$ and define
\begin{equation}
  \label{eq:def_Y_ell}
\bar{g}_{\ell} = g - \pi(g_{\ell}) \eqsp, \quad   Y_{\ell} = \bar{g}_{\ell}(X_\ell) \eqsp,
\end{equation}
so that $S_n = \sum_{\ell =0}^{n-1} Y_{\ell}$.  Note that $\PE_{\pi}[\abs{Y_{\ell}}^{2q}] < \infty$  for any $\ell \in\{0,\ldots,n-1\}$ and therefore $\PE_{\pi}[|S_n|^{2q}] < \infty$. For $u \in \{1,\ldots,q\}$ and $(k_1, \ldots , k_u) \in \{1, \ldots, 2q \}^u$, let $\bk_u = (k_1, \ldots, k_u)$, $|\bk_u| = \sum_{p=1}^u k_p$ and $\bk_u! = \prod_{p=1}^u k_p!$. By the Leonov-Shiraev formula \cite[Eq.~1.53]{saulis:statulevicius:1991}
\begin{equation}
    \PE_\pi[|S_n|^{2q}] = \sum_{u=1}^{2q} \frac{1}{u!} \sum_{|\bk_u| = 2q} \frac{(2q)!}{{\boldsymbol k_u}!} \prod_{p=1}^u \Gamma_{\pi, k_p}(S_n) \eqsp,
\end{equation}
where by \cite[Eq.~1.47]{saulis:statulevicius:1991} for any $k \in \{1,\ldots,2q\}$,
\begin{equation}
  \label{eq:gamma_k_S_n_simple_cumulant}
  \bigl|\Gamma_{\pi,k}(S_n)\bigr| = \bigl|\sum_{0 \le t_1, \ldots, t_k \le n-1} \Gamma_{\pi}(Y_{t_1}, \ldots, Y_{t_k})\bigr| \leq k! \sum_{0\leq t_1 \leq \cdots \leq t_k \leq n-1} \bigl|\Gamma_{\pi}(Y_{t_1}, \ldots, Y_{t_k})\bigr| \eqsp.
\end{equation}
Note that since $i \in \nset$, $\Gamma_{\pi}(Y_i) = \PE_{\pi}[Y_i] = 0$, the expression above simplifies to
\begin{equation}
\label{eq:qmomentexpansion}
     \PE_\pi[|S_n|^{2q}] = \momentGq[q] \{ \PVar[\pi](S_n) \}^q + \sum_{u=1}^{q-1} \frac{1}{u!} \sum_{|\bk_u| = 2q} \frac{(2q)!}{{\boldsymbol k_u}!} \prod_{p=1}^u \Gamma_{\pi, k_p}(S_n) \eqsp.
\end{equation}

To obtain a bound on $\Gamma_\pi(Y_I)$ with $I = (t_1, \ldots, t_k)\in \{0,\ldots,n-1\}^{k}$, $t_1 \leq \dots\leq t_{k}$, we use \eqref{eq:cumulantsviamoments} combined with the following lemma.
\begin{lemma}
\label{lem:centred_moments_markov_property}
Suppose that Assumption \ref{assG:kernelP_q} holds and the Markov kernel $\MK$ has a unique invariant distribution $\pi$, such that $\pi(V) < \infty$. Let $k \in \{1,\ldots,2q\}$ and for any $i \in \{1,\ldots,k\}$, consider $h_i \in \mrl_{V^{p_i/(2q)}}$, $p_i \geq 1$ satisfying  $\sum_{i=1}^k p_i \le 2q$. For any $k$-tuple $(t_1,\dots,t_{k}) \in \{0,\ldots,n-1\}^{k}$, $t_1 \leq \dots\leq t_{k}$, it holds
 \begin{equation}
   \PEC_\pi[h_1(X_{t_1}), \ldots, h_{k}(X_{t_{k}})] = \PEC_\pi[h_1(X_{t_1}), \ldots , h_{k-1}(X_{t_{k-1}}) \tilde h_{k}(X_{t_{k-1}})] \eqsp,
  \end{equation}
  where $\tilde h_{k}(x) = \MK^{t_{k} - t_{k-1}} h_{k}(x) - \pi(h_{k})$.
\end{lemma}
\begin{proof}
Let $\mathfrak F_{k-1} = \sigma\{X_{t_1}, \ldots, X_{t_{k-1}}\}$. By \eqref{eq:def_centered_moment}, we have
\begin{equation}
  \label{eq:def_centered_moment_lem}
     \PEC_{\pi}[h_1(X_{t_1}), \ldots, h_{k}(X_{t_{k}}) ] = \PE_\pi[h_1(X_{t_1}) Z_{2}],
\end{equation}
where $Z_{k+1} = 1$ and for $\ell= 2, \dots, k$, the variables are defined recursively $Z_{\ell} = h_\ell(X_{t_\ell}) Z_{\ell+1} - \PE_\pi[ h_\ell(X_{t_\ell}) Z_{\ell+1}]$. By the tower property, we get for any $\ell \in \{1, \ldots, k-2\}$,
\begin{equation}
\label{eq: tilde z and z}
 \PE_\pi[h_{\ell}(X_{t_{\ell}}) Z_{\ell+1}] = \PE_\pi[h_{\ell}(X_{t_{\ell}})  \PE[Z_{\ell+1}| \mathfrak F_{k-1}]] \eqsp.
\end{equation}
Therefore setting  $\tilde Z_\ell = \PE[Z_{\ell}| \mathfrak F_{k-1}]$, we obtain
\begin{equation}
\label{eq: tilde z_0}
    \tilde Z_\ell  = h_\ell(X_{t_\ell}) \tilde Z_{\ell+1} - \PE_\pi[ h_\ell(X_{t_\ell}) \tilde Z_{\ell+1}] \eqsp.
\end{equation}
For $\ell = k-1$ taking into account that $Z_{k+1} = 1$ and $\PE[h_{k}(X_{t_{k}}) - \pi(h_k) | \mathfrak F_{k-1}] = \tilde h_k(X_{t_{k-1}})$,
\begin{align}
\nonumber
\tilde Z_{k-1} &= h_{k-1}(X_{t_{k-1}}) \PE[h_{k}(X_{t_{k}}) - \pi(h_k)|\mathfrak F_{k-1}]] \\
\nonumber
& \phantom{h_{k-1}(X_{t_{k-1}}) xxxxxx}
- \PE_{\pi}[ h_{k-1}(X_{t_{k-1}}) \PE[h_{k}(X_{t_{k}}) - \pi(h_k) | \mathfrak F_{k-1}] \\
& = h_{k-1}(X_{t_{k-1}}) \tilde h_{k}(X_{t_{k-1}})  - \PE_\pi[ h_{k-1}(X_{t_{k-1}}) \tilde h_{k}(X_{t_{k-1}})] 
\label{eq: tilde z_1}
\eqsp.
\end{align}
We finally set
\begin{equation}
\label{eq: tilde z_2}
\tilde Z_k = 1 \eqsp.
\end{equation}
By the definition of centred moments, $\PEC_\pi[h_1(X_{t_1}), \ldots , h_{k-1}(X_{t_{k-1}}) \tilde h_{k}(X_{t_{k-1}})]$ may be recursively defined via
\begin{equation}
    \PEC_\pi[h_1(X_{t_1}), \ldots , h_{k-1}(X_{t_{k-1}}) \tilde h_{k}(X_{t_{k-1}})] = \PE_\pi[h_1(X_{t_1}) \tilde Z_{2}] \eqsp,
\end{equation}
where $(\tilde Z_\ell)_{\ell = 2}^{k}$ follows \eqref{eq: tilde z_0}, \eqref{eq: tilde z_1} and \eqref{eq: tilde z_2}. Equations~\eqref{eq:def_centered_moment_lem} and \eqref{eq: tilde z and z} with $\ell=1$ implies the statement of the lemma.
\end{proof}

\begin{proof}[Proof of \Cref{th:Rosenthal_w_contracting}]
We give a bound for $\PE[|S_n|^{2q}]$ and then apply \Cref{lem:changeofmeasure_W}. Denote the second term in the r.h.s. of~\eqref{eq:qmomentexpansion} by $R_{\pi, n}$, i.e.
\begin{equation*}
    R_{\pi, n} = \sum_{u=1}^{q-1} \frac{1}{u!} \sum_{|\bk_u| = 2q} \frac{(2q)!}{{\boldsymbol k_u}!} \prod_{p=1}^u \Gamma_{\pi, k_p}(S_n) \eqsp.
\end{equation*}
Since  $\Gamma_{\pi,1}(S_n) = 0$ we may consider the case of $k_p \geq 2, p = 1, \ldots, u$, only. Denote $E_{q, u} = \{\bk_u = (k_1, \ldots, k_u): |\bk_u| = 2q, k_p \geq 2, p = 1, \ldots, u\}$.
Applying Lemma~\ref{lem:cumulants} we get
\begin{equation*}
\begin{split}
|R_{\pi,n}|  &\leq (2 c_m \pi(V))^{2q} \sum_{u=1}^{q-1} \frac{(2q)!}{u!} G_{n,q}^{u} M_q^{2(q-u)} \biggl(\frac{1}{\rho}\biggr)^{u} \biggl(\frac{2}{\log{1/\rho}}\biggr)^{2q-u} \sum_{E_{q,u}} \prod_{i=1}^u (k_i!)^2 \\   
&\le (2 c_m \pi(V))^{2q}  \sum_{u=1}^{q-1} B_{u,q} G_{n,q}^{u} M_q^{2(q-u)},
\end{split}
\end{equation*}
where $B_{u,q}$ is defined in~\eqref{eq: B_u_q_def}. This inequality concludes the statement of the theorem.
\end{proof}


\subsection{Proof of Proposition~\ref{prop:wasser:geo} \label{sec:proof-ros_W_q}}
\begin{proof}
Let $\gamma = p/2q$ and set $\beta = \alpha \gamma$ and assume that $n = km$. It is straightforward to check that $\MKK^m$ satisfies the geometric drift condition
    \begin{equation}
    \label{eq:geometric-drift-condition_m}
    \MKK^m \bar{V} \leq \bar{\lambda}_m \bar{V} + b_m \indi{\bar{C}} \eqsp.
    \end{equation}
    For $\delta  \geq 0$, set $\bar{V}_{\delta}=\bar{V}+\delta$ and
  \begin{align*}
    \tilde{\rho}_{\alpha,\beta, \delta} = \sup_{x,y \in \msx} \left[(1-\epsilon \indi{\bar{C}}(x,y))^{1-\alpha} \left( \frac{K^m\bar V^{\beta/\alpha}_\delta(x,y)}
    {\bar{V}^{\beta/\alpha}_\delta(x,y)}\right)^{\alpha}\right] \eqsp ,
  \end{align*}
  which is finite since $\MKK^m$ satisfies~\eqref{eq:geometric-drift-condition_m}. Furthermore, H\"older's inequality  yields
  \begin{align*}
    \MKK^m(\metricc^{1-\alpha} \bar{V}_\delta^\beta)
    & \leq (\MKK^m\metricc)^{1-\alpha} (\MKK^m\bar V^{\beta/\alpha}_\delta)^\alpha \\
    & \leq \left[(1-\epsilon \indi{\bar C})^{1-\alpha} \left({\MKK^m\bar V^{\beta/\alpha}_\delta}/{\bar{V}^{\beta/\alpha}_\delta}\right)^{\alpha} \right]
      \metricc^{1-\alpha} \bar{V}^\beta_\delta \leq \tilde{\rho}_{\alpha,\beta, \delta} \metricc^{1-\alpha} \bar{V}_\delta^\beta \eqsp.
  \end{align*}
  Using $\bar{V} \leq \bar{V}_\delta$ and a straightforward induction, we obtain for any $k \geq 1$
  \begin{equation}
    \label{eq:wasser:geo:K_n}
    \MKK^{mk} (\metricc^{1-\alpha} \bar V^\beta)\leq \MKK^{mk} (\metricc^{1-\alpha} \bar V_\delta^\beta) \\
    \leq \tilde{\rho}_{\alpha,\beta, \delta}^k \metricc^{1-\alpha} \bar {V}_\delta^\beta\eqsp.
  \end{equation}
  Let $n = k m + \ell, 0 < \ell \le m-1$. H\"older's inequality  yields
  \begin{equation*}
  \begin{split}
    \MKK^\ell(\metricc^{1-\alpha} \bar{V}_\delta^\beta)
    & \leq (\MKK^\ell\metricc)^{1-\alpha} (\MKK^\ell\bar V^{\beta/\alpha}_\delta)^\alpha \\
    & \leq \vartheta^{m(1 - \alpha)} (1 + b/(1-\lambda) + \delta)^{\alpha \gamma}  \metricc^{1-\alpha} \bar V^{\alpha \gamma} \eqsp. 
    \end{split} 
  \end{equation*}
  Together with~\eqref{eq:wasser:geo:K_n}  this inequality implies
  \begin{equation*}
      \MKK^n(\metricc^{1-\alpha} \bar{V}_\delta^\beta) \leq \tilde{\rho}_{\alpha,\beta, \delta}^k \MKK^\ell(\metricc^{1-\alpha}\bar {V}_\delta)^\beta) \le \tilde{\rho}_{\alpha,\beta, \delta}^k \vartheta^{m(1 - \alpha)} (1 + b/(1-\lambda) + \delta)^{\alpha \gamma}  \metricc^{1-\alpha} \bar V^{\alpha \gamma} \eqsp.  
  \end{equation*}
It remains to show that $\tilde{\rho}_{\alpha,\beta,\delta} \leq \rho_{\alpha, \delta}^\gamma$, where $\rho_{\alpha,\delta}$ is given by
\begin{equation}
      \label{eq:def:rho_0}
      \rho_{\alpha,\delta}=\left[(1-\epsilon)^{1-\alpha} \left(\frac{\bar \lambda_m+b_m+\delta}{1+\delta}\right)^\alpha\right]
      \vee \left(\frac{\bar \lambda_m \bar{d}+\delta}{\bar{d}+\delta}\right)^\alpha\eqsp.
    \end{equation}
 Applying~\eqref{eq:geometric-drift-condition_m} we obtain
  \begin{equation}
    \label{eq:wasser:geo:third}
    \frac{\MKK^m\bar V^{\beta/\alpha}_\delta}{\bar V^{\beta/\alpha}_\delta} \leq \{ \varphi(\bar{V}) \}^{\beta/\alpha} \indi{\bar{C}} + \{\psi(\bar{V}) \}^{\beta/\alpha} \indi{\bar{C}^c} \eqsp,
  \end{equation}
  with $\varphi(v) = (\bar{\lambda}_m  v + b_m + \delta)/(v+\delta), \psi(v)= (\bar{\lambda}_m  v   + \delta)/(v+\delta)$. Since $\bar{V} \geq \indi{\bar C} +\bar{d}\indi{\bar C^c}$, we get
  \begin{align*}
    \frac{\MKK^m\bar V^{\beta/\alpha}_\delta}{\bar V^{\beta/\alpha}_\delta} \leq
      \left\{\frac{\bar{\lambda}_m+b_m+\delta}{1+\delta} \right\}^{\beta/\alpha} \indi{\bar C}
    + \left\{\frac{\bar{\lambda}_m + \bar{d}+\delta}{\bar{d}+\delta} \right\}^{\beta/\alpha}  \indi{\bar C^c}\eqsp.
  \end{align*}
  Combining with \eqref{eq:wasser:geo:third} yields
  \begin{equation*}
    (1-\epsilon \indi{\bar C})^{1-\alpha} \left({\MKK^m\bar{V}^{\beta/\alpha}_\delta}/{\bar{V}^{\beta/\alpha}_\delta}\right)^{\alpha}
    \leq \left[(1-\epsilon)^{1-\alpha} \left(\frac{\bar \lambda_m+
          b_m+\delta}{1+\delta}\right)^\beta\right]\indi{\bar C} + \left(\frac{\bar \lambda_m \bar{d}+\delta}{\bar{d}
        +\delta}\right)^\beta \indi{\bar C^c}\eqsp.
  \end{equation*}
  Finally, since $\tilde{\rho}_{\alpha,\beta,\delta}$ is the supremum of the left-hand side over $\msx^2$, we obtain
  that $\tilde{\rho}_{\alpha,\beta,\delta} \leq\rho_{\alpha,\delta}^\gamma$. We choose $\delta = \delta_{\alpha}$ satisfying~\eqref{eq: delta def}. Such $\delta_{\alpha}$ exists since the l.h.s. in~\eqref{eq: delta def} is an increasing function and the r.h.s. is decreasing.
\end{proof}

To simplify notations we will often omit index $\alpha$. We use notations $V_{q} = V^{\alpha/2q}, \bar V_{q} = \bar V^{\alpha/2q}$ and $\rho_{q} = \rho_{\alpha}^{1/2q}$. Let also $\vartheta_q = \vartheta_\alpha^{1/2q}$. 
Furthermore,  let
\begin{equation*}
\Nnorm[q, p, V]{f} := \max \bigg\{\sup_{x \neq x' \in \msx^2} \frac{|f(x) - f(x')|}{\metricc^{1-\alpha}(x,x') \bar V_{q}^{p}(x,x')} , \, \sup_{x \in \msx} \frac{|f(x)|}{V_q^{p}(x)} \bigg\} \eqsp.
\end{equation*}
and $\mathcal{L}_{q, p, V} := \{f: \msx \to \rset: \Nnorm[q, p V]{f} < \infty\}$.  If $q = 1$ we simply write $\Lclass_{q,V}$ and $\Nnorm[q, V]{f}$.
\begin{lemma}
\label{lem: P^n h class}
Let Assumptions \ref{assG:kernelP_q} and \ref{assG:kernelP_q_contractingset_m} hold. For any $h \in \Lclass_{q, p, V}$ with $\pi(h) = 0$, and $n \in \nset$, $\MK^n h \in \Lclass_{q, p, V}$ with $\Nnorm[q, p, V]{\MK^n h} \leq 2 \kappa \{\vartheta_{\alpha} \pi(V^\alpha)\}^{p/(2q)}  \Nnorm[q, p, V]{h} \rho_{\alpha}^{pn/(2q)}$.
\end{lemma}
\begin{proof}
Eq.~\eqref{eq: constraction}  implies
\begin{equation}
\begin{split}
    |\MK^n h(x) - \MK^n h(y)| &\le \int K^n(x,y, \rmd x' \rmd y') |h(x') - h(y')| \\
    & \le \Nnorm[q, p, V]{h} \int \MKK^n(x,y, \rmd x' \rmd y') \metricc^{1-\alpha}(x',y') \bar V_{q}^p(x',y') \\
    & \le \kappa \Nnorm[q, p, V]{h} \vartheta_{q}^p \rho_{\alpha}^{pn/(2q)} \bar V_{q}^{p}(x,y)\eqsp.
    \end{split}
\end{equation}
Moreover, integrating with respect to $\pi$ we get
\begin{equation}
\begin{split}
    | \MK^n h(x)  - \pi(h)| 
    &\leq \Nnorm[q, p, V]{h} \vartheta_{q}^p  \rho_{\alpha}^{pn/(2q)} \int \bar V_q^p(x,y) \pi(\rmd y) \\
    &\leq 2 \kappa \{\vartheta_{\alpha} \pi(V^\alpha)\}^{p/(2q)}  \Nnorm[q, p, V]{h} \rho_{\alpha}^{pn/(2q)} V_{q}^p(x) \eqsp.
    \end{split}
\end{equation}
\end{proof}

\begin{lemma}
\label{lem: product of two funct}
Let $h_i \in \Lclass_{q, p_i, V}$ for $i = 1,2$. Then $h_1 h_2 \in \Lclass_{q, p_1 + p_2, V}$ and $\Nnorm[q, p_1+p_2, V]{h_1 h_2} \le 4 \Nnorm[ q, p_1, V]{h_1}  \Nnorm[q, p_2, V]{h_2}$.
\end{lemma}
\begin{proof}
Fix any $x, y \in \msx$. Then
\begin{equation*}
\begin{split}
      |h_1(x) h_2(x) - h_1(y) h_2(y)| &\le |h_1(x) - h_1(y)||h_2(x)| + |h_2(x) - h_2(y)||h_1(y)| \\
      & \le \Nnorm[q, p_1, V]{h_1} \metricc^{1-\alpha}(x,y) \bar V_{ q}^{p_1}(x,y) \Nnorm[q, p_2, V]{h_2} V_{q}^{p_2}(x) \\
      & + \Nnorm[q, p_2, V]{h_2} \metricc^{1-\alpha}(x,y) \bar V_{q}^{p_2}(x,y) \Nnorm[q, p_1, V]{h_1} V_{q}^{p_1}(y) \eqsp.
    \end{split}
\end{equation*}
Since $V(x) \le 2\bar{V}(x,y)$ we get
\begin{equation*}
 |h_1(x) h_2(x) - h_1(y) h_2(y)| \le 2^{ 1 + \alpha(p_1+p_2)/(2q)} \Nnorm[q, p_1, V]{h_1}  \Nnorm[q, p_2, V]{h_2} \metricc^{1-\alpha}(x,y) \bar V_{q}^{p_1+ p_2}(x,y) \eqsp.
\end{equation*}
Similarly,
\begin{equation*}
    |h_1(x) h_2(x)| \le \Nnorm[q, p_1, V]{h_1}  \Nnorm[q, p_2, V]{h_2} V_{q}^{p_1 + p_2}(x)  \eqsp.
\end{equation*}
The last two inequalities imply the statement.
\end{proof}

\begin{lemma}
\label{lem:centered_moments_W}
Let Assumptions \ref{assG:kernelP_q} and \ref{assG:kernelP_q_contractingset_m} hold.  Let $k \in \nset$, $k \leq 2q$, and $h_i \in \Lclass_{q, p_i, V}$, $i \in \{1, \dots, k\}$, be arbitrary functions such that $\pi(h_i) = 0$ and $\sum p_i \le 2q$, $p_i \geq 1$. For any ordered $k$-tuple $T=(t_1,\dots,t_{k}) \in \{0,\ldots,n-1\}^{k}$, $t_1 \le \ldots \le t_k$,
\begin{equation}
\label{eq:centred_moments-1}
  |\PEC_\pi[h_1(X_{t_1}), \ldots, h_k(X_{t_k})] | \le \pi(V_q^{p_1+\ldots+p_k
  }) (8 \kappa)^{k}  \ConstC_{q}^{M(p_1, \ldots, p_k)} \rho_{q}^{t_k - t_1} \prod_{\ell = 1}^k    \Nnorm[p_\ell, V]{h_\ell}
\end{equation}
where $m_{\ell}^k = \sum_{j = \ell}^k p_j$ and $M(p_1, \ldots, p_k) = \sum_{\ell=2}^k m_{\ell}^k$.
\end{lemma}
\begin{proof}
  We proceed by induction. For $k = 1$ the statement is obvious since $\pi(h_1) = 0$.  Assume that~\eqref{eq:centred_moments-1} holds for $k$. By Lemma \ref{lem:centred_moments_markov_property}
  \begin{equation}
   \PEC_\pi[h_1(X_{t_1}), \ldots, h_k(X_{t_k}) h_{k+1}(X_{t_{k+1}})] = \PEC_\pi[h_1(X_{t_1}), \ldots , h_k(X_{t_k}) \tilde h_{k+1}(X_{t_k})],
  \end{equation}
  where $
  \tilde h_{k+1}(x) = P^{t_{k+1} - t_k} h_{k+1}(x)$.
  Since $h_{k+1} \in \Lclass_{q, p_{k+1}, V}$, we get by Lemma \ref{lem: P^n h class} that $\tilde h \in \Lclass_{q, p_{k+1}, V}$ with $\Nnorm[q, p_{k+1}, V]{\tilde h_{k+1}} \le 2 \kappa \ConstC_{q}^{p_{k+1}}  \Nnorm[ q, p_{k+1}, V]{h}  \myrho{\alpha}{\bar d}{q}^{t_{k+1} - t_{k}}$.
  Hence, by Lemma~\ref{lem: product of two funct}
  $$
  \Nnorm[q, p_k+p_{k+1}, V]{h_k \tilde h_{k+1}} \le 8 \kappa \ConstC_{q}^{p_{k+1}} \myrho{\alpha}{\bar d}{q}^{t_{k+1} - t_{k}}  \Nnorm[q, p_k, V]{h_1}  \Nnorm[q, p_{k+1}, V]{h_2} \eqsp.
  $$
\end{proof}

\begin{Corollary}
\label{coro:centered_moments_wasserstein}
Suppose that Assumption~\ref{assG:kernelP_q}--\ref{assG:kernelP_q_smallset} hold.  Let $q \in \nset$, $u,k \in \{1,\ldots,q\}$ and for any $i \in \{1,\ldots,k\}$, consider $h_i \in \mrl_{V^{p_i/(2q)}}$, $p_i \geq 1$ satisfying  $\pi(h_i) = 0$, $\sum_{i=1}^k p_i \leq u$. Then for any $k$-tuple $I = (t_1,\dots,t_{k}) \in \{0,\ldots,n-1\}^{k}$, $t_1 \leq \dots\leq t_{k}$ it holds
\begin{equation}
\label{eq:centred_moments_one_Z_new}
  |\PEC_\pi[h_1(X_{t_1}), \ldots, h_k(X_{t_k})]| 
  \leq 2^k (c_m \pi(V))^{ku/q} \rho^{\maxgap(I)/2} \prod_{\ell = 1}^k   \|h_\ell\|_{V^{p_{\ell}/(2q)}} \eqsp,
\end{equation}
where $\maxgap(I) := \max_{j \in \{2,\dots,k\}}[t_{j}-t_{j-1}]$.
\end{Corollary}

\begin{lemma}
\label{lem:changeofmeasure_W}
Let Assumptions \ref{assG:kernelP_q} and \ref{assG:kernelP_q_contractingset_m} hold and $q \in [1,\infty)$. Let $(g_{\ell})_{\ell = 0}^{n-1} \in \Lclass_{q,V}$. Then, for any probability measure $\xi$ such that $\xi(V)<\infty$,
\begin{equation*}
     \PE_\xi\big[ \big|S_n \big|^{2q} \big] \le \rme \PE_\pi\big[ \big|S_n \big|^{2q} \big]
      + \vartheta_q^{2q} M_q^{2q} (2q+1)^{2q} \left( \xi(V^\alpha) + \pi(V^\alpha) \right) (1 - \myrho{\alpha}{\bar d}{q})^{-2q}  \eqsp.
\end{equation*}
\end{lemma}
\begin{proof}
 Applying inequality $(a+b)^{2q}
\le \rme a^{2q}+ (1 + 2q)^{2q} b^{2q}$ for $a \geq 0, b \geq 0$, we obtain
\begin{equation*}
\PE_{\xi}\big[\big|S_n \big|^{2q}
\big] \leq  \rme \PE_\pi \big[ \big|S_n|^{2q}\big] + (1 + 2q )^{2q} \PE_{\xi \otimes \pi}\bigg[ \bigg| \sum_{i=0}^{n-1} \bar g_i(X_i) -\bar g_i(X'_i) \bigg|^{2q}\bigg]  \eqsp.
\end{equation*}
Then, by the Minkowski's inequality we obtain
\begin{equation*}
\bigg\{\PE_{\xi \otimes \pi}\bigg[ \bigg| \sum_{i=0}^{n-1} \bar g_i(X_i) - \bar g_i(X'_i) \bigg|^{2q}
\bigg] \bigg\}^{1/2q} \le  \sum_{i=0}^{n-1} \{ \PE_{\xi \otimes \pi}[|  \bar g_i(X_i) - \bar g_i(X'_i) |^{2q}\}^{1/2q}
 \eqsp.
\end{equation*}
Applying $|\bar g_i(x) - \bar g_i(x')| \leq  \Nnorm[q,V]{\bar g_i} \metricc^{1-\alpha} (x,x')\bar V_q(x,x')$ for any $(x,x') \in \msx^2$, $\metricc(x,x') \le 1$ and \eqref{eq: constraction} we obtain
\begin{equation}
    \begin{split}
     \{ {\PE}_{\xi \otimes \pi}[|  \bar g_i(X_i) - \bar g_i(X'_i) |^{2q} \}^{1/2q} &\leq
\Nnorm[q,V]{\bar g_i}  \{ {\PE}_{\xi \otimes \pi}[\metricc^{1-\alpha} (X_i,X_i') \bar{V}^{\alpha}(X_i,X'_i)] \}^{1/2q} \\
& \le  \myrho{\alpha}{\bar d}{q}^{i}  \vartheta_{q}  \Nnorm[q,V]{\bar g_i} \bigg\{\int \bar V^\alpha(x,y) \pi(\rmd y) \xi(\rmd x) \bigg\}^{1/2q} \\
& \le \myrho{\alpha}{\bar d}{q}^{i}  \vartheta_{q}  \Nnorm[q,V]{\bar g_i} \{ \xi(V^\alpha) + \pi(V^\alpha) \}^{1/2q} \eqsp.
    \end{split}
\end{equation}
This formula implies
\begin{equation*}
        \sum_{i=0}^{n-1} \{ \PE_{\xi \otimes \pi}[|  g_i(X_i) - g_i(X'_i) |^{2q} \}^{1/2q} \leq \vartheta_{q} \left(  \xi(V^\alpha) + \pi(V^\alpha) \right)^{1/2q} \sum_{i=0}^{n-1}\|\bar g_{i}\|_{V^{1/(4q)}} \myrho{\alpha}{\bar d}{q}^{i} \Nnorm[q,V]{\bar g_i}\eqsp.
\end{equation*}
We conclude the proof by noting that $\Nnorm[q,V]{\bar g_i} \le M_q$.
\end{proof}



\subsection{Technical lemmas}
%upper bounds for A and B
\begin{lemma}
\label{lem:A_B_bound}
Let $B_{u,q}$ be an expression defined in \eqref{eq: B_u_q_def}. Then, for any $k \geq 2$, $0 < \rho < 1$, and $1 \leq u \leq q-1$, it holds
\begin{equation}
\label{eq:B_upper_bound}
\begin{split}
B_{u,q} \leq \biggl(\frac{\rme q}{q-u}\biggr)^{q-u} \biggl(\frac{\rme (2q-u-1)}{2q-2u}\biggr)^{2q-2u} \bigl((2q-2u+2)!\bigr)^2 \biggl(\frac{2}{\log{1/\rho}}\biggr)^{2q}\biggl(\frac{2\log{1/\rho}}{\rho}\biggr)^{u}\eqsp.
\end{split}
\end{equation}
\end{lemma}
\begin{proof}
%To obtain \eqref{eq:A_upper_bound}, it is enough to note that 
%\[
%(r+1)^{k-2}\rho^{r/2} \leq \frac{1}{\rho} \int_{r+1}^{r+2}x^{k-2}\rho^{x/2}\,\rmd x\eqsp.
%\] 
Using \eqref{eq: B_u_q_def},
\begin{align*}
B_{u,q} 
&\leq \frac{q!}{u!}\sum_{k_1 + \ldots + k_u = 2q, k_i \geq 2}  \prod_{i=1}^u (k_{i}!)k_i A_n(k_{i}, \rho) \\
&\leq \frac{q!}{u!} \biggl(\frac{2}{\log{1/\rho}}\biggr)^{2q-u}\biggl(\frac{1}{\rho}\biggr)^{u}\sum_{k_1 + \ldots + k_u = 2q, k_i \geq 2}  \prod_{i=1}^u (k_{i}!)^2 \\
&\leq \frac{q!}{u!} \biggl(\frac{2}{\log{1/\rho}}\biggr)^{2q-u}\biggl(\frac{1}{\rho}\biggr)^{u} \binom{2q-u-1}{u-1} \bigl((2q-2u+2)!\bigr)^2 2^{2u-2}\eqsp.
\end{align*}
In the last inequality we used the fact that number of integer solutions to $k_1 + \ldots + k_u = 2q, k_i \geq 2$ is $\binom{2q-u-1}{u-1}$. Now the final upper bound follows from elementary inequalities
\begin{align*}
&\frac{q!}{u!} = \binom{q}{q-u}(q-u)! \leq \biggl(\frac{\rme q}{q-u}\biggr)^{q-u}\eqsp, \\
&\binom{2q-u-1}{u-1} = \binom{2q-u-1}{2q-2u} \leq \biggl(\frac{\rme (2q-u-1)}{2q-2u}\biggr)^{2q-2u}\eqsp.
\end{align*}
\end{proof}


==> Technical.tex <==
\begin{lemma} 
\label{lem:bsum}
Let $a > 0$ and $(\alpha_k)_{k \geq 0}$ be a non-increasing sequence such that $\alpha_0 < 1/a$. Then
\[
\sum_{j=0}^{n+1} \alpha_j \prod_{l=j+1}^{n+1} (1 - \alpha_l a) = \frac{1}{a} \left\{1  - \prod_{l=1}^{n+1} (1 - \alpha_l a) \right\}
\]
\end{lemma}
\begin{proof}
Let us denote $u_{j:n+1} = \prod_{l = j}^{n+1} (1 - \alpha_l a)$. Then, for $j \in\{1,\dots,n+1\}$,
$u_{j+1:n+1} - u_{j:n+1} = a \alpha_j u_{j+1:n+1}$. Hence,
\[
\sum_{j=0}^{n+1} \alpha_j \prod_{l=j+1}^{n+1} (1 - \alpha_l a) = \frac{1}{a} \sum_{j=1}^{n+1} (u_{j+1:n+1} - u_{j:n+1}) = a^{-1} ( 1 - u_{1:n+1} ) \,.
\]
\end{proof}

\begin{lemma}
\label{lem:bsum2}
Let $b > 0$ and $(\alpha_k)_{k \geq 0}$ be a non-increasing sequence such that $\alpha_0 < 1/(2b)$.
\begin{itemize}
    \item Assume $\alpha_k - \alpha_{k+1} \le \smallConst{\alpha} \alpha_{k+1}^2$ with $\smallConst{\alpha} \le b/2$. Then for $p \in (1, 2]$,
    \[
\sum_{k=1}^{n+1} \alpha_k^{p} \prod_{j=k+1}^{n+1}(1 - b \alpha_j) \le (2/b) \alpha_{n+1}^{p-1}.
\]
    \item 
    Assume $\alpha_k - \alpha_{k+1} \le \smallConst{\alpha} \alpha_{k+1}^2$,   $\alpha_k/\mathcal A_{k+1} \le (2/3)\smallConst{\alpha}$  with $\smallConst{\alpha} \le b/4$. We additionally assume that $\alpha_0 \le (2 \smallConst{\alpha})^{-1}$. Then for any $p \in (1,2], q \in [0,1]$
\[
\sum_{k=1}^{n+1} \alpha_k^p \mathcal A_{k}^q \prod_{j=k+1}^{n+1}(1 - b) \alpha_j) \le (2/b) \alpha_{n+1}^{p-1}\mathcal A_{n+1}^{q}.
\]
\end{itemize}

\end{lemma}
\begin{proof}
For the first part 
\begin{align*}
&\sum_{k=1}^{n+1} \alpha_k^{p} \prod_{j=k+1}^{n+1}(1 - b \alpha_j) = \alpha_{n+1}^{p-1} \sum_{k=1}^{n+1} \alpha_k \prod_{j=k+1}^{n+1} \bigg(\frac{\alpha_{j-1}}{\alpha_j} \bigg)^{p-1}  (1 - b \alpha_j) \\
&\qquad\qquad\qquad \le \sqrt{\alpha_{n+1}} \sum_{k=1}^{n+1} \alpha_k \prod_{j=k+1}^{n+1} (1 + \smallConst{\alpha}\alpha_j) (1 - b \alpha_j) \\
&\qquad\qquad\qquad \le \alpha_{n+1}^{p-1} \sum_{k=1}^{n+1} \alpha_k \prod_{j=k+1}^{n+1} (1 - (b/2) \alpha_j) \le (2/b) \alpha_{n+1}^{p-1},
\end{align*}
where on the last step we used \Cref{lem:bsum}. For the second part, we first note that
$$
\frac{\mathcal A_{j-1}}{\mathcal A_j} \le 1 + \frac{\alpha_{j-1}^2}{\mathcal A_j} \le 1 + (2/3)\smallConst{\alpha} \alpha_{j-1} \le 1 + (2/3) \smallConst{\alpha} \alpha_j + (2/3) \smallConst{\alpha}^2 \alpha_j^2 \le 1 + \smallConst{\alpha} \alpha_j.
$$
Similarly to the first part,
\begin{align*}
&\sum_{k=1}^{n+1} \alpha_k^p \mathcal A_{k}^q\prod_{j=k+1}^{n+1}(1 - b \alpha_j) = \alpha_{n+1}^{p-1} \mathcal A_{n+1}^q\sum_{k=1}^{n+1} \alpha_k \prod_{j=k+1}^{n+1} \bigg(\frac{\alpha_{j-1}}{\alpha_j} \bigg)^{p-1} \bigg(\frac{\mathcal A_{j-1}}{\mathcal A_j} \bigg)^q  (1 - b \alpha_j) \\
&\qquad\qquad\qquad \le \alpha_{n+1}^{p-1} \mathcal A_{n+1}^q \sum_{k=1}^{n+1} \alpha_k \prod_{j=k+1}^{n+1} (1 + \smallConst{\alpha}\alpha_j)^2 (1 - b \alpha_j) \\
&\qquad\qquad\qquad \le \alpha_{n+1}^{p-1} \mathcal A_{n+1}^q\sum_{k=1}^{n+1} \alpha_k \prod_{j=k+1}^{n+1} (1 - (b/2) \alpha_j) \le (2/b) \alpha_{n+1}^{p-1}\mathcal A_{n+1}^{q},
\end{align*}
where we also used Lemma~\ref{lem:bsum}.
\end{proof}




==> foo.tex <==
\subsection{An illustrative example}
In this section, we derive the statement of ... for a specific example
and justify such a form. More precisely, we show that if $\alpha >0$
is fixed, there exists $\bar{p}>0$ such that
$\lim_{n \to \plusinfty} \PE[\normLigne{\theta_n-\thetas}^p] =
\plusinfty$ for $p \geq \bar{p}$. As a result, typical Gaussian or
even exponential concentration bounds for $(\theta_n)_{n \in \nset}$ is not possible.
The particular example that we consider here consists in the one-dimensional instantiation of \eqref{eq:lsa} taking for
  $(Z_k)_{k \in\nset}$ an \iid~sequence of tilde Rademacher with parameter $q \in
  \ooint{1/2,1}$:
\begin{equation}
  \label{eq:particular_example}
  Z_k =
  \begin{cases}
    1 & \text{ with probability $q$}\eqsp, \\
    -1 & \text{ with probability $1-q$}\eqsp,
  \end{cases}
  \quad \text{ and $A(z) = z, b(z) = 0$, for $z \in \{-1,1\}$ } \eqsp.
\end{equation}
This choice is associated with $\thetas = 0$ and corresponds to the recursion:
\begin{equation}
  \label{eq:particular_example_2_old}
  \theta_n = \prod_{k=1}^n (1-\alpha Z_k) \theta_0 \eqsp, \qquad \theta_0 \in \rset \eqsp.
\end{equation}
Define
\begin{equation}
  \varphi_q(\alpha) =   q \log\parenthese{\frac{1+\alpha}{1-\alpha}} - \log(1+\alpha)  \quad \text{ and } \balpha_q = \sup \{\balpha >0 \, : \,  \varphi_q(\alpha) >0 \text{ for any } \alpha \in \ooint{0,\balpha}\} \eqsp.
\end{equation}
Note that $\varphi_q(\alpha) \in\ccint{0,1}$ for $\alpha >0$ and $  \varphi_q(\alpha) \sim  \alpha(2 q-1)$ as $\alpha \to 0$. Therefore since $q > 1/2$, $\{\balpha >0 \, : \,  \varphi_q(\alpha) >0 \text{ for any } \alpha \in \ooint{0,\balpha}\} \not = \emptyset$ and  $\balpha_q$ is well-defined.
% \begin{equation}
%   \label{eq:3}
%   q \log\parenthese{\frac{1+\alpha}{1-\alpha}} - \log(1+\alpha) =0 \eqsp.
% \end{equation}
\begin{proposition}
  \label{propo:particular_example}
  Consider $(\theta_n)_{n \in \nset}$ defined by \eqref{eq:particular_example_2} with $\theta_0 =1$ and $\alpha \in \ooint{0,\balpha_q}$. Then, for any $\delta \in \ccint{\rme^{-2n\varphi_q(\alpha)},1}$, it holds
  \begin{equation*}
     \proba{\theta_n \geq \exp\parenthese{- \varphi_q(\alpha) n  + \log\parenthese{\frac{1+\alpha}{1-\alpha}}\sqrt{n\log(1/\delta)/2}}} \leq \delta \eqsp.
  \end{equation*}
\end{proposition}

\begin{proof}

Let $\alpha \in \ooint{0,\balpha_q}$. First we write \eqref{eq:particular_example_2} as
\begin{equation*}
\theta_n  = (1-\alpha)^{N_n}(1+\alpha)^{n-N_n} \eqsp, \quad \text{ where $N_n = \sum_{k=1}^n \1_{\{1\}}(Z_k)$ } \eqsp.
\end{equation*}
Then, for any $\beta >0$, we get
\begin{align}
  \nonumber
  \proba{\theta_n \geq \rme^{-\alpha \beta n }} &= \proba{\log (\theta_n) \geq - \alpha \beta n } = \proba{N_n \log\parenthese{\frac{1-\alpha}{1+\alpha}} \geq -\alpha\beta n - n \log(1+\alpha)}
  \\
    \nonumber
                                           & = \proba{N_n \leq n \log^{-1}\parenthese{\frac{1+\alpha}{1-\alpha}}\defEns{\alpha \beta + \log(1+\alpha)}} \\
  \label{eq:particular_example_3}
                                           &   = \proba{N_n -qn  \leq -n \parentheseDeux{q- \log^{-1}\parenthese{\frac{1+\alpha}{1-\alpha}}\defEns{\alpha \beta + \log(1+\alpha)}}} \eqsp.
\end{align}

Let $  \beta_{\alpha,q} = \alpha^{-1} \parentheseDeux{q \log\defEns{(1+\alpha)/(1-\alpha)} - \log(1+\alpha)}$,
% \begin{equation}
%   \label{eq:def_beta_limit}
%  \beta_{\alpha,q} = \alpha^{-1} \parenthese{q \log\parenthese{\frac{1+\alpha}{1-\alpha}} - \log(1+\alpha)}   \eqsp.
% \end{equation}
Note that with the condition, $\alpha\in\ooint{0,\balpha_q}$, $\beta_{\alpha,q} >0$ and therefore for any $\beta \in\ccint{0,\beta_{\alpha,q}}$,
\begin{equation}
  x_{\alpha,\beta}  = \parentheseDeux{q- \log^{-1}\parenthese{\frac{1+\alpha}{1-\alpha}}\defEns{\alpha \beta + \log(1+\alpha)}} \in \ccint{0,\varphi_q(\alpha)} \eqsp,
\end{equation}
It follows using Hoeffding's inequality that for any $\beta \in\ccint{0,\beta_{\alpha,q}}$,
\begin{equation}
\label{eq:ineq_proba_theta_n}
  \proba{\theta_n \geq \rme^{-\alpha \beta n }}    \leq \rme^{-2n x_{\alpha,\beta}^2}\eqsp.
\end{equation}
% Using a Taylor expansion, we have
% \begin{equation*}
% \log^{-1}\parenthese{\frac{1+\alpha}{1-\alpha}} \sim (2\alpha)^{-1}(1+o(\alpha)) \eqsp,
% \end{equation*}
% and therefore
% we get that
% \begin{equation}
%   \label{eq:2}
%   \beta_{\alpha,q} \sim 2q-1 + \alpha/2 \eqsp.
% \end{equation}
Let $\delta \in \ccint{\bdelta_{q,\alpha},1}$. Therefore, there exists $x \in \ocint{0,\varphi_q(\alpha)}$ such that $\rme^{-2n x_{\alpha,\beta}^2} = \delta$ given by $x_{\alpha,\beta} = \sqrt{\log(1/\delta)/2n}$, which corresponds to
\begin{equation*}
 \beta  = \alpha^{-1} \{q-\sqrt{\log(1/\delta)/2n}\}\log\parenthese{\frac{1+\alpha}{1-\alpha}} -\log(1+\alpha)  \in\ccint{0,\beta_{\alpha,q}} \eqsp.
\end{equation*}
This completes the proof using \eqref{eq:ineq_proba_theta_n}.
\end{proof}

\begin{proposition}
  \label{propo:1}
  Consider $(\theta_n)_{n \in \nset}$ defined by \eqref{eq:particular_example_2} with $\theta_0 =1$. Then, for any $p \geq 1$ and $\alpha \in\ooint{0,1}$,
  \begin{equation*}
    \PE\parentheseDeux{\abs{\theta_n}^p} \geq \{1-p\alpha[(2q-1) -(p-1)\alpha(1-q)/2]\}^n \eqsp.
  \end{equation*}
\end{proposition}

\begin{proof}
 Let $p \geq 1$ and $\alpha \in\ooint{0,1}$. First note that by definition \eqref{eq:particular_example_2}, we have that
    \begin{equation*}
    \PE\parentheseDeux{\abs{\theta_n}^p} \geq \{q(1-\alpha)^p+(1-q)(1+\alpha)^p \}^n \eqsp.
  \end{equation*}
The proof is then a simple consequence of the lower bounds $(1-\alpha)^p \geq 1-\alpha p$ and $(1+\alpha)^p \geq 1+\alpha p  + p(p-1)\alpha^2/2$.
\end{proof}
Note that if $\alpha \in \ooint{0,1}$ is fixed, then for $p > \bar{p}_{q,\alpha} = 1+2(2q-1)/[\alpha(1-q)]$, $\lim_{n\to \plusinfty}     \PE\parentheseDeux{\abs{\theta_n}^p} = \plusinfty$.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../neurips_paper"
%%% End:


==> impossibility-results.tex <==
To simplify the problem, we consider the case $d=1$, $\theta_0=0$, and $\bar{A}(Z_t), \bar{b}(Z_t)$ are i.i.d. (and $\bar{A}(Z_t)$ independent of $\bar{b}(Z_t)$). Even in this simple setting, the iterates $\theta_t$ and $\bar{\theta}_t$ explode with non-negligible probability. More precisely, the iterates reach values in $e^{aT}$ with probability larger than $e^{-bT}$ for $a,b>0$, typical of heavy-tailed distributions. This makes it impossible for a bound w.h.p. to hold without a non-logarithmic dependence on $\delta$, or exponential dependence in $T$.

First, note that Eq.~(\ref{eq:lsa}) directly implies
\begin{equation}
\theta_T = \sum_{t=1}^T \prod_{i=t+1}^T (I - \alpha A_i) \alpha b_t + \prod_{i=1}^T (I - \alpha A_i) \theta_0\,.
\end{equation}
Let $\varepsilon > 0$, $p=\P(\bar{A}(Z_1) < -\varepsilon / \alpha)$ and $q = \P(\bar{b}(Z_1) > \varepsilon / \alpha)$. If $\bar{A}(Z_t)$ and $\bar{b}(Z_t)$ are not bounded almost surely, then $pq > 0$, and we have
\begin{equation}
\P\left(\theta_T \geq \sum_{t=1}^T (1+\varepsilon)^{T-t} \varepsilon\right) = \P\left(\theta_T \geq (1+\varepsilon)^T - 1\right) \geq (pq)^T\,.
\end{equation}

Hence, if we have, $\forall T\geq 0$ and $\forall\delta > 0$, \begin{equation}
\P\left(\bar{\theta}_T \geq f(T,\delta)\right) \leq \delta\,,
\end{equation}
then, $\forall T\geq 0$,
\begin{equation}
f\left(T, (pq)^T\right) \geq \frac{(1+\varepsilon)^T - 1}{(T+1)}\,,
\end{equation}
and the bound $f(T,\delta)$ is either non-logarithmic (e.g. polynomial) in $\delta$ or exponential in $T$.

\subsection{General case ($d>1$)}
For any $\varepsilon,\eta > 0$, let
\begin{equation}
p_\varepsilon = \max_{u\in\mathbb{R}^d} \min_{v\in\mathbb{R}^d} \P(u^\top (\varepsilon I + \bar{A}(Z_1)) v \leq 0)\,,
\end{equation}
and
\begin{equation}
q_\eta = \min_{v\in\mathbb{R}^d} \max\left\{\P(v^\top \bar{b}(Z_1) \geq \eta\|v\|), \P(v^\top \bar{b}(Z_1) \leq -\eta\|v\|) \right\}\,.
\end{equation}

Then, with probability at least $(p_\varepsilon q_\eta)^T$, there exists $u\in\mathbb{R}^d$ such that $\|u\|=1$ and, for all $t\in\{0,\dots,T-1\}$,
\begin{equation}
u^\top\theta_{t+1} = u^\top(I-\alpha \bar{A}(Z_{t+1}))\theta_t + \alpha u^\top\bar{b}(Z_{t+1}) \geq (1 + \alpha\varepsilon)u^\top\theta_t + \alpha\eta\,,
\end{equation}
and thus
\begin{equation}
u^\top\theta_t \geq \left(\frac{\eta}{\varepsilon} + u^\top\theta_0\right) (1+\alpha\varepsilon)^t - \frac{\eta}{\varepsilon}\,.
\end{equation}
Finally, using $\bar{\theta}_T = \frac{1}{T}\sum_{t=0}^{T-1}\theta_t$, we have
\begin{equation}
u^\top\bar{\theta}_T \geq \left(\frac{\eta}{\varepsilon} + u^\top\theta_0\right) \frac{(1+\alpha\varepsilon)^T - 1}{\alpha\varepsilon T} - \frac{\eta}{\varepsilon}\,.
\end{equation}

\begin{lemma}
Let $\theta^*\in\mathbb{R}^d$. If $\forall T\geq 1$ and $\forall\delta > 0$, $\P\left(\sqrt{T}\|\bar{\theta}_T - \theta^*\| \geq f(T,\delta)\right) \leq \delta$, then, $\forall T\geq 1$,
\begin{equation}
f\left(T, (p_\varepsilon q_\eta)^T\right) \geq \sqrt{T}\left[\left(\frac{\eta}{\varepsilon} + u^\top\theta_0\right) \frac{(1+\alpha\varepsilon)^T - 1}{\alpha\varepsilon T} - \frac{\eta}{\varepsilon} - u^\top\theta^*\right]\,.
\end{equation}
\end{lemma}

\begin{Corollary}
Let $\varepsilon > 0$, $\theta^*\in\mathbb{R}^d$, and assume that $\forall T,\delta > 0$, $\P\left(\sqrt{T}\|\bar{\theta}_T - \theta^*\| \geq f(T,\delta)\right) \leq \delta$. Then, if $p_\varepsilon > 0$, there exists $\theta_0\in\mathbb{R}^d$ such that
\begin{equation}
% \max_{T\leq 1} f\left(T, \delta\right) \geq \sqrt{\ln(1/p_\varepsilon q_\eta)}\left(\frac{\eta}{\varepsilon} + u^\top\theta_0\right) \frac{\delta^{\ln(1+\alpha\varepsilon)/\ln(p_\varepsilon q_\eta)} - 1}{\alpha\varepsilon \sqrt{\ln(1/\delta)}} - \sqrt{\frac{\ln(1/\delta)}{\ln(1/p_\varepsilon q_\eta)}}\left(\frac{\eta}{\varepsilon} - u^\top\theta^*\right)\,.
\max_{T\geq 1} f\left(T, \delta\right) = \Omega\left( \frac{\delta^{-\ln(1+\alpha\varepsilon)/\ln(2/p_\varepsilon)}}{\sqrt{\ln(1/\delta)}}\right)\,.
\end{equation}
\end{Corollary}

\begin{lemma}
Let $p,\varepsilon > 0$, $\bar{A}\in\mathbb{R}^{d\times d}$, and $X\in\mathbb{R}$ a positive random variable. Then, there exists a random matrix $A\in\mathbb{R}^{d\times d}$ such that $\mathbb{E}[A] = \bar{A}$ and
\begin{equation}
p_\varepsilon = \P\left( X \geq \min_u \|(\varepsilon I + \bar{A})u\| \right) \mbox{ and } \max_{u\in\mathbb{S}^{d-1}} \mathbb{E}\left[ \|(A - \bar{A})u\|^p \right] = \mathbb{E}\left[ X^p \right]\,.
\end{equation}
\end{lemma}

==> notation.tex <==
\paragraph{Notation}
For arbitrary matrix $B \in \rset^{d \times d}$ we denote by $\sigma_\ell(B), \ell = 1, \ldots, d$, its singular values and denote its Schatten \(p\)-norm by $\norm{B}[p] = \{\sum_{\ell=1}^d \sigma_\ell^p(B)\}^{1/p}$. For $p, q \geq 1$ and random matrix $\X$ we introduce $\norm{\X}[p,q] = \{\PE [\norm{\X}[p]^q] \}^{1/q}$.

